Assessing Centrality Without Knowing Connections

We consider the privacy-preserving computation of node influence in distributed social networks, as measured by egocentric betweenness centrality (EBC). Motivated by modern communication networks spanning multiple providers, we show for the first time how multiple mutually-distrusting parties can successfully compute node EBC while revealing only differentially-private information about their internal network connections. A theoretical utility analysis upper bounds a primary source of private EBC error---private release of ego networks---with high probability. Empirical results demonstrate practical applicability with a low 1.07 relative error achievable at strong privacy budget $\epsilon=0.1$ on a Facebook graph, and insignificant performance degradation as the number of network provider parties grows.

==> TimingResults.tex <==
\begin{figure*}[ht]
\centering
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, Facebook data , for three parties. ]{\label{fig:b}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimefacebook.pdf}
}
\hfill
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, Enron data set , for three parties. ]{\label{fig:e}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimeenron.pdf}
}
\hfill
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, PGP data set, for three parties. ]{\label{fig:h}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimepgpMultipgp.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, Facebook data set.]{\label{fig:c}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1facebook.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, degree, Enron data set.]{\label{fig:f}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1enron.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, PGP data set.]{\label{fig:i}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1PGP.pdf}
}
\caption{Timing results and effect of degree for Facebook, Enron and PGP data sets.}
\label{fig_sim}
\end{figure*}

==> arXiv-Assessing Centrality Without KnowingConnections/TimingResults.tex <==
\begin{figure*}[ht]
\centering
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, Facebook data , for three parties. ]{\label{fig:b}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimefacebook.pdf}
}
\hfill
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, Enron data set , for three parties. ]{\label{fig:e}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimeenron.pdf}
}
\hfill
\subfloat[Time of computing 60 random nodes with $\epsilon=$0.1 to 7, PGP data set, for three parties. ]{\label{fig:h}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiEpsilonVStimepgpMultipgp.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, Facebook data set.]{\label{fig:c}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1facebook.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, degree, Enron data set.]{\label{fig:f}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1enron.pdf}
}
\hfill
\subfloat[Relative error of 60 nodes with different degrees for $\epsilon=$1, PGP data set.]{\label{fig:i}\includegraphics[width=0.32\textwidth, keepaspectratio]{MultiDegreeVSrelativeerrorep1PGP.pdf}
}
\caption{Timing results and effect of degree for Facebook, Enron and PGP data sets.}
\label{fig_sim}
\end{figure*}

==> arXiv-Assessing Centrality Without KnowingConnections/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
